On Charge 3 Symmetric Monopoles

Monopoles are solutions of an SU(2) gauge theory in $\mathbb{R}^{3}$ satisfying a lower bound for energy and certain asymptotic conditions, which translate as topological properties encoded in their charge. Using methods from integrable systems, monopoles can be described in algebraic-geometric terms via their {spectral curve}, i.e. an algebraic curve, given as a polynomial P in two complex variables, satisfying certain constraints. In this thesis we focus on the Ercolani-Sinha formulation, where the coefficients of P have to satisfy the Ercolani-Sinha constraints, given as relations amongst periods. A particular class of such monopoles is studied, namely charge 3 monopoles with a symmetry by $C_{3}$, the cyclic group of order 3. This class of cyclic 3-monopoles is described by the genus 4 spectral curve $\hat{X}$, subject to the Ercolani-Sinha constraints: the aim of the present work is to establish the existence of such monopoles, which translates into solving the Ercolani-Sinha constraints for $\hat{X}$.

==> monopoles.tex <==
\introcap{We give here some background about monopoles. After a short overview of the original differential geometric formulation, we briefly present the Nahm and Hitchin descriptions, which are more algebraic-geometric in flavour; within this setting we introduce symmetric monopoles, which are a main theme of this work. We then describe the Ercolani-Sinha formulation, which, using tools from integrable systems, provides a suitable framework for exact monopole solutions: in this context, we examine in some detail a certain symmetric charge 3 monopole studied by Braden and Enolskii.
}

\numberwithin{equation}{section}
\section{A very short introduction to monopoles}
The setting is a \enf{gauge theory}, the prototype of which is electromagnetism. \\
In the geometric formulation of electromagnetism, the fundamental objects are a 1-forms on $\mathbb{R}^3$, the electric field $\el$, and a 2-form on $\mathbb{R}^3$, the magnetic field $\magn$. Out of these, one can build the Maxwell field tensor $\ef=\magn+c\; \de t \wedge \el \;\in\Omega^{2}(\mathcal{M}_{4})$, where  $\mathcal{M}_{4}=\mathbb{R}^3 \times \mathbb{R}$ is the four dimensional Minkowski space-time. In these geometric terms, Maxwell equations (in absence of sources) can be written as follows:
\begin{equation}\label{maxwelleq}
 \de \ef=0,\qquad \de \star \ef=0,
\end{equation}
where $\star$ is the Hodge star. The first of eq. (\ref{maxwelleq}) implies that $\ef$ is closed on $\mathcal{M}_{4}$, hence can be expressed as $\ef=\de \A$, where $\A$ is a 1-form, the vector potential.\\
From its very definition, the vector potential is defined up to an exact form, or in other words  it is invariant under a gauge transformation $\A \to \A+\de \alpha$. Geometrically this means that  $\A$ is a connection form of a (trivial) $U(1)$ bundle over $\mathcal{M}_{4}$, and $\ef$ is its curvature. Note that the setting where the necessity of the bundle description really arises is, in fact, that of the so-called \enf{Dirac monopole} \cite{dirac}. A Dirac monopole is a solution of the Maxwell equation with a magnetic charge at the origin of $\mathbb{R}^3$. The magnetic  field $\magn$ corresponding to such  a magnetic monopole is given by
\begin{equation*}
 \magn = \frac{1}{4\pi r^3}(x_1 \de x_2 \wedge \de x_3 + cyclic).
\end{equation*}
In terms of the ``usual'' vector $\vec{B}$ this would read
\begin{equation*}
 \vec{B}(\mathbf{x})= \frac{\mathbf{x}}{4\pi r^3}
\end{equation*}
where $\mathbf{x}=(x_{1},x_{2},x_{3}),\;r=|\mathbf{x}|$.\\
With this magnetic field, there exists no globally defined form $\A$ such that   $\ef=\de \A$. However, it is possible to find such a form locally, for instance 
\begin{align*}
\A_N=\;\frac{1}{4\pi r} \frac{1-\cos\theta}{\sin\theta} \mathbf{e}_{\phi}\quad \mathrm{on}\quad U_{N}\\
\A_S=-\frac{1}{4\pi r} \frac{1+\cos\theta}{\sin\theta} \mathbf{e}_{\phi}\quad \mathrm{on} \quad U_{S},
\end{align*}
where $U_N=S_N\times\mathbb{R}$ and $U_S=S_S\times\mathbb{R}$, where $S_N$ (resp. $S_S$) is the sphere minus the north (resp. south) pole. 
Thus $\ef=\de \A$ holds locally. Note that the following relation holds:
\begin{equation*}
 \A_N=\A_S+\de\alpha, \qquad \mathrm{where} \; \alpha=-\frac{1}{2\pi}\phi.
\end{equation*}
which is precisely the Maurer-Cartan equation for a connection on a $U(1)$ bundle.\\
In general, the connection viewpoint is extremely powerful  when the space has a nontrivial topology, as in this case, where there is a singularity at the origin. However, in this work we are mostly interested in monopoles without singularities, defined in the whole of $\mathbb{R}^3$: this means that for a connection there is always a globally defined gauge potential. 
Nevertheless, these monopoles share important similarities with the Dirac monopole, including some sort of topological nature.

\subsection{$SU(2)$ monopoles}

Pure Yang-Mills theory is a gauge theory directly modelled on electromagnetism, but with gauge group a non-abelian Lie group instead of $U(1)$. The connection $\A$ is interpreted (in the quantum theory) as giving rise to a vector particle for every generator of the Lie algebra of $G$, with zero mass; in order to incorporate mass in a gauge invariant way, one has to include in the theory a new field $\higgs$, the \enf{Higgs field}.\\The action is then (proportional to)
\begin{equation}\label{actionYM}
 S=\int_{\mathcal{M}}\Big((\ef,\ef)+(\covde \higgs,\covde \higgs)+V(\higgs)\de vol \Big) 
\end{equation}
where $V$ is a gauge invariant potential, $\covde$ is the covariant derivative associated to the connection $\A$,  
and $(\ef,\ef)=\mathrm{Tr}(\ef\wedge \star \ef)$.\\
In the following, we only consider a theory on $\mathbb{R}^3$ equipped with the Euclidean metric, with gauge group $SU(2)$, a Higgs fields taking values in the adjoint bundle to the principal $SU(2)$ bundle on $\mathbb{R}^3$ and zero potential.\\
The action then reads
%
\begin{equation*}
 S=\int_{\mathbb{R}^3}\Big((\ef,\ef)+(\covde \higgs,\covde \higgs)\Big);
\end{equation*}
%
since $S$  is interpreted as the energy of the system, one has to ensure that it is finite. This is achieved by imposing the following field behaviour at infinity\footnote{
Note that this ensures the finiteness of the energy only when the fields satisfy the Bogomolny equations \ref{bogom}.
} 
(for details see \cite{jt}):%
\begin{align}\label{bc1}
\begin{split}
||\higgs||= 1+O(r^{-1})\\
 \frac{\partial ||\higgs||}{\partial \Omega}= O(r^{-2}),\\
 ||\covde \higgs||= O(r^{-2}),
 \end{split}
\end{align}
where $ \frac{\partial }{\partial \Omega}$ denotes the angular derivative (along a sphere).
\\
Integrating the action density over a ball of radius $R$ centered at the origin, one has:
\begin{align}\label{eqb1}
 \int_{B^{2}_{R}}\big(\left(\ef,\ef\right)+\left(\covde \higgs,\covde \higgs\right)\big) &=
\int_{B^{2}_{R}}\big(\left(\ef-\star\covde \higgs,\ef-\star\covde \higgs\right)+2\left(\star\covde \higgs,\ef\right)\big).
\end{align}
Upon using the Bianchi identity for $\ef$:
\begin{align*}
 \de(\higgs,\ef)&%
 =(\star\covde\higgs,\ef),
\end{align*}
which implies that 
\begin{align*}
 \int_{B^{2}_{R}}(\star\covde \higgs,\ef)\;=&\int_{S^{2}_{R}}(\higgs,\ef),
\end{align*}
where $S^{2}_R=\partial B^{2}_{R}$.  Let the connection $\A$ be defined on a rank $2$ vector bundle $E$.  For large $R$, as $||\higgs||\to 1$ by \eqref{bc1}, its eigenspaces define complex line bundles $L$ and $L^{*}$  over $S^{2}_{R}$, with Chern class $\pm k$. 
%
With the decay conditions $||\covde \higgs||= O(r^{-2})$, the projection of the curvature $\ef$ on these line bundles approaches the curvature of the bundles themselves:
%
\begin{equation*}
 \lim_{R\to\infty}\int_{S_{R}}(\higgs,\ef) =\pm 4\pi k,
\end{equation*}
%
hence
\begin{equation*}
 S=\int_{\mathbb{R}^3}(\ef-\star\covde \higgs,\ef-\star\covde \higgs)\;\pm4\pi k.
\end{equation*}
Therefore, if $k \geqslant 0$, the action $S$ is minimised if $(\A,\higgs)$ satisfies the \enf{Bogomolny equations}:
\begin{equation}\label{bogom}
 \ef=\star\covde\higgs.
\end{equation}
A Higgs field solving these equations can in fact be shown to have (in a suitable gauge) the following asymptotic expansion:
\begin{equation*}
\higgs \sim \begin{pmatrix}i & 0 \\ 0 & -i\end{pmatrix} -\frac{k}{2r} \begin{pmatrix}i & 0 \\ 0 & i\end{pmatrix}  +O(r^{-2}).
\end{equation*}
This adds a further constraint to the asymptotic conditions (\ref{bc1}); hence we can now give the following
\begin{definition}
 An \enf{$SU(2)$ monopole of charge $k$} is a solution of the above \enf{Bogomolny equations} with (minimal) energy $4\pi k$ and boundary conditions
 \begin{align}\label{bc}
\begin{split}
 ||\higgs||&= 1-\frac{k}{2r}+O(r^{-2})\\
 \frac{\partial ||\higgs||}{\partial \Omega}&= O(r^{-2}),\\
||\covde \higgs||&= O(r^{-2}),
 \end{split}
\end{align}
\end{definition}

\begin{remark}
We notice that monopoles  also arise as dimensional reduction of a Yang-Mills theory in the four dimensional Euclidean space. More specifically, consider an $SU(2)$ gauge theory on the Euclidean $\mathbb{R}^4$, with Higgs field taking values in the adjoint bundle and action  as in eq. (\ref{actionYM}), with a non zero potential: 
%
\begin{equation}\label{actionYM4}
S=\int_{\mathbb{R}^4}\left((\ef,\ef)+(\covde \higgs,\covde \higgs)+\lambda(1-|\higgs|^2)^2\de^4 x\right)  
\end{equation}
%
 If we  consider only  the solutions which are invariant by translations along, for instance, the fourth coordinate, these can be dimensionally reduced to $\mathbb{R}^3$, where the first three components of $\A$ can be interpreted as components of a connection on $\mathbb{R}^3$, and the fourth as the Higgs field.\\ 
Taking $\lambda=0$ in the potential, and keeping the boundary conditions given by the finiteness of the action \eqref{actionYM4} results in the dimensional reduction of the self-duality equations $\ef=\star\ef$  to the Bogomolny equations (\ref{bogom}).\\
Thus, \enf{$SU(2)$ monopoles} can be interpreted as \enf{static self-dual solutions of Yang-Mills equations on $\mathbb{R}^4$}.
 \end{remark}
 
\begin{remark}
Note that setting $\lambda=0$ in (\ref{actionYM4}) is known (mainly in the physics literature) as taking the BPS limit of the Yang-Mills action. Indeed,  \,'t Hooft and Polyakov found the first monopole solution in a non abelian gauge theory, namely a static solution of the fields equation coming from eq. (\ref{actionYM4}) with $\lambda\neq 0$; their analysis was mainly numerical. Shortly after this, Prasad and Sommerfield found an analytic form for the solution in the case $\lambda=0$, which is a spherically symmetric monopole of charge 1. Then Bogomolny studied further this $\lambda=0$ limit, also  introducing the Bogomolny equations (\ref{bogom}). Hence this class of monopoles is often referred to as BPS monopoles: in this work, we refer to them simply as monopoles.
\end{remark}

\begin{remark}
Finally, we point out that in the case of a gauge group $U(1)$, Bogomolny equations reduce to 
$$B= \mathrm{grad}~\higgs$$ where $\higgs=\frac{k}{2r}$. This corresponds indeed to the Dirac monopole.
\end{remark}


%
%
%
\section{Nahm construction}
% 
The above  description of monopoles, whilst very beautiful, does not prove very useful when finding explicit monopoles solutions. Hence, several different approaches have been developed to this aim, both approximate and exact. In this work we are mainly concerned with Nahm's approach \cite{nahm}, and the subsequent formulations given by Hitchin (\cite{hitmon, hitgeo}), and Ercolani and Sinha (\cite{es}); in this section, we describe Nahm's formulation.\\

In \cite{nahm} Nahm managed to adapt the Atiyah-Hitchin-Drinfeld-Manin (ADHM, see \cite{ADHM}) construction for instantons to the case of monopoles. The equivalence between the geometric description of monopoles and Nahm's algebraic description was proven by Hitchin in \cite{hitmon}, where he also showed the equivalence of yet another formulation, that we refer to as Hitchin's formulation (explained in section \ref{hitchinform}). \\

The crucial construction needed to understand this alternative formulation is the \enf{Nahm transform}, which is a two way transform: it takes solutions of the Bogomolny equations (with boundary conditions (\ref{bc})) to solutions of the Nahm's equations, a first order differential equation between matrices satisfying certain conditions (see end of this section), and vice versa.\\
In analogy to the ADHM construction, Nahm considers a Dirac operator on $\mathbb{R}^{3}$, given by:
\begin{equation*}
\Dirac=\left(
\begin{array}{cc}
    0 & D_{z}   \\
     D^{\dagger}_{z} & 0
\end{array}
\right)=
\left(
\begin{array}{cc}
    0 &\boldsymbol{\sigma}\cdot \covde -(\higgs+iz)  \\
     \boldsymbol{\sigma}\cdot \covde +(\higgs+iz) & 0
\end{array}
\right)
\end{equation*}
where $\boldsymbol{\sigma}=(\sigma_{1},\sigma_{2},\sigma_{3})$ are the Pauli matrices,  $\Dirac$ acts on  $\mathcal{L}^{2}$-normalizable $\mathbb{C}^{2}\times \mathbb{C}^{2}$ valued\footnote{
Both $\mathbb{C}^{2}$s are representations of $\mathfrak{su}(2)$: the first copy is the spin space where the $\sigma_{i}$ act, the other is the space where the connection and the Higgs live.
} 
 functions on $\mathbb{R}^{3}$, and $D^{\dagger}$ is the adjoint of $D$.\\
After using Bogomolny equations, one finds:
\begin{equation*}
D_{z}D^{\dagger}_{z}= \covde \cdot \covde -(\higgs+iz)(\higgs+iz),
\end{equation*}
which means  $D_{z}D^{\dagger}_{z}$ is a positive operator, and hence has no ($\mathcal{L}^{2}$-normalizable) zero modes; this in particular  implies that the $\mathcal{L}^{2}$-kernel of $D^{\dagger}_{z}$ is empty. One can show\footnote{Using an $\mathcal{L}^{2}$ index theorem it follows that $D_{z}$ has an index $k$ if  $z\in(-1,1)$ , and zero otherwise.} that $D_{z}$ has $k$-dimensional $\mathcal{L}^{2}$-kernel $N_{z}$ only if $z\in(-1,1)$ . \\
Consider then an orthonormal basis for $N_{z}$,  namely $k$ functions $\psi^{i}$ such that
\begin{equation*}
D_{z}\psi^{i}=0, \qquad \int_{\mathbb{R}^{3}}(\psi^{i},\psi^{j})=\delta_{ij},
\end{equation*}
and satisfying
\begin{equation*}
\int_{\mathbb{R}^{3}}(\psi^{i},\frac{\partial \psi^{j}}{\partial z})=0.
\end{equation*}
These functions can be used to define the three \enf{Nahm matrices} as follows:
\begin{equation}\label{nahmmatrices}
T^{ij}_{a} (z)=\int_{\mathbb{R}^{3}}(\psi^{i},x_{a}\psi^{j}).
\end{equation}
These matrices satisfy a number of properties,  given below.
%
\begin{itemize}
\item[\nuno] \enf{Nahm equations}: 
\begin{equation}\label{nahmeq}
\frac{\de T_{i}}{\de t}=\frac{1}{2}\sum_{j,k} \varepsilon_{ijk}[T_{j},T_{k}].
\end{equation}
%
\item[\ndue] $T_{i}$ is analytic for $z\in(-1,1)$ and has simple poles at $z=-1$, $z=1$, where the residues form irreducible $k$-dimensional representations of $\mathfrak{su}(2)$.
%
\item[\ntre] $\qquad T_{i}(z)=-T_{i}^{{\dagger}}(z)  \qquad T_{i}(z)=T_{i}^{T}(-z)$.
%
\end{itemize}

A proof of these properties can be found either in Nahm's paper \cite{nahm}, or in the review \cite{wy}.\\


%
A solution of eqs. \eqref{nahmeq} satisfying conditions \nuno, \ndue , \ntre\, can be mapped back to a connection and a Higgs field via the inverse Nahm transform, which has a similar structure to the map introduced earlier, and is given schematically as follows (for details see again \cite{nahm} or  \cite{wy}).\\
Consider the differential operator
\begin{equation*}
D_{x}:=\frac{\de}{\de z} - T_{i}\sigma^{i}-x_{j}\sigma_{j}. 
\end{equation*}
It can be shown that its $\mathcal{L}^{2}$-kernel $E_{x}$ is 2-dimensional (this makes use of \ndue). Choosing an orthonormal basis\footnote{Note that the ambiguity in the choice of this basis is reflected in an ambiguity in the definition (\ref{nahmfields}) of the fields up to a gauge transformation} $(v_{1},v_{2})$ for $E_{x}$, define a connection and a Higgs field by
\begin{align}\label{nahmfields}
\begin{split}
\higgs_{ab}&=i\int_{-1}^{1} z v^{\dagger}_{a}(z)v_{b}(z) \de z,\\
\A_{ab}&=i\int_{-1}^{1} z v^{\dagger}_{a}(z)\frac{\partial}{\partial x_{i}}v_{b}(z) \de z.
\end{split}
\end{align}
$\A$ and $\higgs$ so defined are indeed smooth solutions of the Bogomolny equations with the appropriate boundary conditions for a charge $k$ monopole.\\
We can then state the following theorem.
\begin{theorem}[\enf{Nahm \cite{nahm}, Hitchin \cite{hitmon}}]
An \enf{$SU(2)$ monopole of charge $k$}, namely a solution of the Bogomolny equations with (minimal) energy $4\pi k$ and boundary conditions (\ref{bc}), is equivalent to a solution of the \enf{Nahm equations} \nuno, subject to the conditions \ndue, \ntre.
\end{theorem}\vspace{3mm}


\begin{remark}
The Nahm transform and its inverse are isometries, and the Nahm transform followed by its inverse gives back the original monopole.
\end{remark}\vspace{2mm}
%
\begin{remark}
Nahm's equations can be cast in \enf{Lax form}, which allows to use methods from integrable systems; we explain  this in some more detail.\\
Define
\begin{align*}
A_{-1}&=(T_{1}+iT_{2}), &  A_{0}&=-2iT_{3} , &  A_{1}=T_{1}-iT_{2},
\end{align*}
and hence, introducing a \enf{spectral parameter} $\zeta\in\puno$:
\begin{align*}
A&=A_{-1}\zeta^{-1}+A_{0}+A_{1}\zeta,    &  M&=\frac{1}{2}A_{0}+A_{1}\zeta.
\end{align*}
Then \nuno\; becomes
\begin{equation*}
\frac{\de A}{\de z}=[A,M],
\end{equation*}
\ie  a \enf{Lax form for Nahm's equations}. This permits to use integrable system methods to find a solution to Nahm's equations. Indeed, an algebraic curve appears, namely the \enf{spectral curve}, given by the equation (see Chapter \ref{intsys})
\begin{equation}\label{nahmcurve}
P(\zeta,\eta)=\mathrm{det}(\eta\mathbb{I}-A)=
\mathrm{det}\left(\eta+(T_{1}+iT_{2})-2iT_{3}\zeta+(T_{1}-iT_{2})\zeta^{2}\right)=0,
\end{equation}
and Nahm's equations describe a linear flow on the Jacobian on this curve. As described in Chapter \ref{intsys}, there are (almost) algorithmic approaches to deal with this class of systems:  in particular, in this work we make use of the finite-gap integration method, due to Krichever (see section \ref{krth} for more details), in a framework due to Ercolani and Sinha (see \cite{es} and section \ref{esform}). 
\end{remark}\vspace{2mm}
%
%
% 
\begin{remark}
Finally, it has been possible to solve Nahm's equations in a number of nontrivial cases, and then to carry out the inverse Nahm transform, at least numerically: in this way a number of monopole solutions of different charges  have been constructed explicitly; this has proven useful especially to describe qualitative features of monopoles, such as the energy density distribution.\\
\end{remark}

%
%
\section{Hitchin data}\label{hitchinform}
Another approach to monopoles in terms of a certain class of holomorphic bundles on $\tang\puno$ is given by Hitchin; here we only sketch very briefly this construction, referring to \cite{hitgeo} for details.\\

The idea is to consider the set of oriented geodesics on $\mathbb{R}^{3}$ with the Euclidean metric, which is in fact isomorphic to $\tang\puno$; a solution to the Bogomolny equations gives rise to a holomorphic bundle on this surface.\\

To set notation, introduce homogeneous coordinates $[\zeta_{0}:\zeta_{1}]$  on $\puno = U_{0} \cup U_{1}$, with $U_{i}$ standard open sets. Let $\zeta=\zeta_{0}/\zeta_{1}$ be a coordinate on $U_{0}$; hence  standard coordinates $(\zeta,\eta)$ on $\pi^{-1}(U_{0})\subset  \tang\puno$ are defined by $(\zeta,\eta)\to \eta\dfrac{\de}{\de \zeta}$ (and similarly for $U_{1}$).\\
With respect to these coordinates and the open covering of $\tang\puno$ given by $\tilde{U}_{i}=\pi^{-1}(U_{i})$, the line bundle $L^{j}$ is defined by the transition function $\exp(-j\tfrac{\eta}{\zeta})$ in the intersection $\tilde{U}_{0}\cap\tilde{U}_{1}$.\\
Recall that in $\puno$  the transition function $g_{01}=\zeta^{n}$ on $U_{0}\cap U_{1}$ defines the line bundle $\OO(n)$ (which is the unique line bundle of degree $n$ on $\puno$); denote the pullback of this line bundle to $\tang\puno$ also by $\OO(n)$. Take then the tensor product of  this line bundle $\OO(n)$ with the line bundle $L^{j}$ defined earlier, to obtain the bundle $L^{j}(n):= L^{j}\otimes\OO(n) $.\\


Consider the differential operator:
\begin{equation*}
D_{\gamma}=\covde_{\gamma}-i\higgs,
\end{equation*}
where $\covde_{\gamma}$ is the covariant derivative along the oriented straight line $\gamma$.\\
Define a bundle $\tilde{E}$ on the space of geodesics by associating to each $\gamma$ the (2-dimensional) kernel  $E_{\gamma}$ of $D_{\gamma}$. If $\A$ and $\higgs$ satisfy the Bogomolny equations, one can endow $\tilde{E}$ with a \emph{holomorphic structure} (with some additional properties, see Theorem 4.2 in \cite{hitgeo}).\\
The bundle $\tilde{E}$ has two holomorphic sub-bundles, $E^{\pm}$, whose fibers $E^{\pm}_{\gamma}$ are solutions of $D_{\gamma}f=0$ which decay at $\pm\infty$ along the line $\gamma$. It can be seen (Theorem 6.3 in \cite{hitgeo}) that $E^{+}\simeq L(-k)$ and $E^{-}\simeq L^{*}(-k)$.%
The set of those curves $\gamma$ for which $E^{+}_{\gamma}= E^{-}_{\gamma}$ forms a curve in $\tang\puno$, called the \enf{spectral curve}  $S$ of the monopole. Since a decaying solution decays exponentially, the spectral curve is also the set of lines along which there is an $\mathcal{L}^{2}$-solution.\\
One can give a more precise characterisation of the spectral curve. That the quotients of $\tilde{E}$ by $E^{\pm}$ satisfy $$\tilde{E}/E^{+}\simeq L(k),\qquad \tilde{E}/E^{-}\simeq L^{*}(k).$$
The curve $S$ is defined by the vanishing of the map $E^{+}\to \tilde{E}/E^{-}$ and hence by a section of $(E^{+})^{*}\otimes  \tilde{E}/E^{-} \simeq \mathcal{O}(2k) $. In terms of the standard coordinates  $(\zeta,\eta)$ on $\tang\puno$, $S$ is then defined by an equation of the form:
 \begin{equation}\label{hcurve}
 P(\eta,\zeta)=\eta^{k}+a_{1}(\zeta)\eta^{k-1}+\ldots +a_{k-1}(\zeta)\eta+a_{k}(\zeta),
 \end{equation}
where $a_{j}(\zeta)$, $0\leq j\leq k$ are polynomial of degree at most $2j$ in $\zeta$.\\
This curve satisfies the following properties (\cite{hitgeo, hitmon})
\begin{itemize}

\item[\textbf{H0}]   $S$ is compact and has no multiple components.
\item[\huno] \enf{Reality condition}: the curve $S$ is invariant under the standard real structure $\tau$ on $\tang\puno$. The involution $\tau$ is defined by reversing the orientation of the lines in $\mathbb{R}^{3}$, and in coordinates takes the following form
\begin{equation}\label{realstr}
\tau:(\zeta,\eta) \rightarrow \left(-\dfrac{1}{\bar{\zeta}},-\dfrac{\bar{\eta}}{\bar{\zeta}^{2}}\right).
\end{equation}
This invariance condition translates to the following relations amongst the coefficients $a_{i}$
\begin{equation*}
a_{j}(\zeta)=(-1)^{j}\zeta^{2j}\overline{a_{j}\left(-\frac{1}{\bar{\zeta}}\right)}.
\end{equation*}
%
%
\item[\hdue] $L^{2}$ is holomorphically trivial on $S$ and $L(k-1)$ is real.\\
The first statement follows from the fact that, on $S$, $E^{+}$ and $E^{-}$ are isomorphic, which is equivalent to say that $E^{+}\otimes E^{-}\;(\simeq L^{2})$. Both these properties are consequences of the boundary conditions (\ref{bc}).
\item[\htre] $H^{0}(S,L^{s}(k-2))=0$ for $s\in(0,2)$. This is equivalent to the non-singularity of the monopole determined by $S$.
%
\end{itemize}
%
The above findings can be summarised  in the following theorem.
\begin{theorem}[\enf{Hitchin \cite{hitmon}}]\label{hitthm}
An \enf{$SU(2)$ monopole of charge $k$}, namely a solution of the Bogomolny equations with (minimal) energy $4\pi k$ and boundary conditions (\ref{bc}), is equivalent to a spectral curve of the form (\ref{hcurve}), subject to the \enf{Hitchin conditions \huno,  \hdue, \htre}.
\end{theorem}
%
Incidentally,  note that from the above properties one can deduce, using Riemann-Hurwitz formula, that the genus of $S$ is $g_{S}=(k-1)^{2}$.\\

%
If $k=1$, the spectral curve (\ref{hcurve}) satisfying \huno, \hdue, \htre\; takes the form :
\begin{equation}\label{kuno}
\eta=(x_{1}+ix_{2})-2x_{3}\zeta-(x_{1}-ix_{2})\zeta^{2},
\end{equation}
where $(x_{1},x_{2},x_{3})=\mathbf{x}\in\mathbb{R}^{3}$ and can be interpreted as the \enf{centre} of the monopole; indeed, such a curve is the set of all oriented lines through the point $\mathbf{x}$. This curve is also called a \emph{real section} as it defines a real section of the bundle $\tang\puno\to\puno$.\\
A $k$-monopole also has a well defined centre (as well as a total phase), whose coordinates $(c_{1},c_{2},c_{3})$  enter in the spectral curve as coefficients of the polynomial $a_{1}(\zeta)$ as follows:
\begin{equation}\label{a1center}
a_{1}(\zeta)=(c_{1}+ic_{2})-2c_{3}\zeta-(c_{1}-ic_{2})\zeta^{2},
\end{equation}\vspace{2mm}

%
\begin{center}
\begin{minipage}{350pt}
\enf{Note}:  Nahm's  and Hitchin's approaches are indeed equivalent: this is shown in the fundamental paper \cite{hitmon}, where a link among these two formulations, and the original geometric description is given. We remark that both in Hitchin's and in Nahm's data an algebraic curve appears, directly as in $\huno$, or indirectly as in eq. (\ref{nahmcurve}): this is indeed the \enf{same curve} in two different manifestations.
\end{minipage}\vspace*{5mm}
\end{center}
%
%
%
\section{Symmetric Monopoles}\label{symmmon}
%
Although the methods outlined above provide a great deal of simplification, in general it proves quite involved to find an exact solution for a monopole, and not many solutions have been found thus far: a notable exception is the case of \enf{symmetric monopoles}. Symmetric monopoles are $k$-monopole solutions which are \enf{invariant under various symmetries}:  this constrains their spectral curves, and in some cases it is quite immediate to infer the non-existence of monopoles with certain symmetries. It is more difficult to obtain results on the existence and on the exact form of the solutions, although some solutions have been found already in the early paper \cite{symmmon}. The  fundamental paper \cite{symmmon} is the basis for the exposition below: we have chosen to present this topic in Hitchin formalism, rather than in Nahm formalism because, despite using the latter in most of this thesis, we believe that symmetry is more natural and transparent in the former. \\

A general monopole curve has the form given in eq. (\ref{hcurve}), subject to conditions \huno, \hdue, \htre; here we investigate the form of these curves when the monopole is required to be invariant with respect to certain symmetry groups of $\mathbb{R}^{3}$ of \enf{rotations around the origin}. To implement this symmetry, the  monopole is taken to be centered at the origin, which means, from eq. (\ref{a1center}), that $a_{1}(\zeta)=0$. But before doing this,  a special type of symmetry, namely \enf{inversion}, is discussed.

\subsection{Inversion}
The inversion map in $\mathbb{R}^{3}$ is the reflection in the $(x_{1},x_{2})$ plane, namely:
\begin{equation*}
I:(x_{1},x_{2},x_{3})\longrightarrow (x_{1},x_{2},-x_{3}).
\end{equation*}
As this map reverses orientation, it induces an anti-holomorphic map on the space $\tang\puno$, which in standard coordinates reads
\begin{equation*}
\phi:\; (\zeta,\eta) \rightarrow \left(\dfrac{1}{{\bar{\zeta}}}, -\dfrac{\bar{\eta}}{\bar{\zeta}^{2}}\right) 
\end{equation*}
%
Notice that $\phi$ is very similar to the real structure $\tau$ of eq. (\ref{realstr}); in fact $$\phi\circ\tau(\zeta,\eta)= (-\zeta,\eta).$$
It follows then that if $P(\zeta,\eta)=0$ is a monopole curve, and hence invariant under $\tau$, then the inverted curve is $P(-\zeta,\eta)=0$.\\
It is interesting to study the monopoles which are invariant under inversion; in particular, their moduli space presents an interesting structure (see \cite{symmmon}, section 4). Moreover, they form a large class, and  are also easy to characterise: their spectral curve is given by polynomials $P(\zeta,\eta)=0$ which are \emph{even} in $\zeta$.

%
%
%
%
%
\subsection{Rotations}\label{symmrotcurv}
Let us now recall that an $SO(3)$ rotation in $\mathbb{R}^{3}$ corresponds to a M\"{o}bius transformation in $\puno$ and hence $\tang\puno$. In particular, a rotation by an angle $\theta$ around the unit vector $(n_{1},n_{2},n_{3})$ is represented in $\tang\puno$ as :
\begin{align*}
\zeta \to \zeta' =\dfrac{(d+ic)\zeta+(b-ia)}{-(b+ia)\zeta+(d-ic)}, \qquad 
\eta \to \eta'  =\frac{\eta}{\left(-(b+ia)\zeta+(d-ic)\right)^{2}}
\end{align*}
where
\begin{equation*}
n_{1}\sin\frac{\theta}{2}=a,\quad  
n_{2}\sin\frac{\theta}{2}=b,\quad
n_{3}\sin\frac{\theta}{2}=c,\quad
\cos\frac{\theta}{2}=d,\quad
\end{equation*}
%
Thus, a monopole is invariant under a rotation if its spectral curve $P(\zeta,\eta)=0$ is invariant under the associated M\"{o}bius transformation, namely $P(\zeta',\eta')=0$ is the same curve. One can then examine the consequences of invariance under a number of uncomplicated subgroups of $SO(3)$.\\

\begin{example}[\enf{Cyclic and dihedral monopoles}]
The first simple example is the \enf{cyclic group of rotations $C_{n}$} around the $x_{3}$ axis. It is generated by
\begin{equation*}
\zeta'=\e^{\tfrac{2\pi i}{n}}\zeta, \qquad \eta'=\e^{\tfrac{2\pi i}{n}}\eta.
\end{equation*}
Hence, for $P(\zeta,\eta)=0$ to be invariant under $C_{n}$, all terms must have the same total degree, $mod$ $n$; since the leading term is $\eta^{k}$, all terms must have degree $k$ $mod$ $n$. In particular, for $P(\zeta,\eta)=0$ to be invariant under $C_{k}$, all terms must have degree $0$, $mod$ $k$.\\

The groups $C_{n}$ are extended to \enf{dihedral groups} $D_{n}$ by adding to the generators a rotation by $\pi$ around the $x_{1}$-axis, which corresponds to the transformation:
\begin{equation}\label{extrasymm}
\zeta'=\frac{1}{\zeta},\quad \eta'=-\frac{\eta}{\zeta^{2}}.
\end{equation}
%
%
%


Let us consider some examples of such symmetric curves, namely charge $3$ monopoles with either $C_{3}$ or $D_{3}$ symmetry. A general charge 3 monopole curve takes the form
\begin{align*}\begin{split}
\eta^{3}+\eta&(\alpha_{4}\zeta^{4}+\alpha_{3}\zeta^{3}+\alpha_{2}\zeta^{2}+\alpha_{1}\zeta^{1}+\alpha_{0})+\\
\qquad &(\beta_{6}\zeta^{6}+\beta_{5}\zeta^{5}+\beta_{4}\zeta^{4}+\beta_{3}\zeta^{3}+\beta_{2}\zeta^{2}+\beta_{1}\zeta^{1}+\beta_{0})=0,
\end{split}\end{align*}
where the coefficients are subject to the following conditions:
\begin{align*}
\alpha_{4}&=\bar{\alpha}_{0}, &\alpha_{3}&=\bar{\alpha}_{1},& \alpha_{2}&=\bar{\alpha}_{2}; & \; &\\
\beta_{6}&=-\bar{\beta}_{0},& \beta_{5}&=\bar{\beta}_{1},& \beta_{4}&=-\bar{\beta}_{2}, &\beta_{3}&=\bar{\beta}_{3}.
\end{align*}
%
%
Imposing the $C_{3}$ symmetry, the curve reduces to
\begin{equation}\label{c3curve}
\eta^{3}+\alpha\eta\zeta^{2}+\beta\zeta^{6}+\gamma\zeta^{3}-\bar{\beta}=0,
\end{equation}
where $\alpha,\gamma\in\mathbb{R}$, and also $\beta$ can be made real by a change of coordinates (rotation about the $x_{3}$-axis).\\

Imposing on (\ref{c3curve}) the extra symmetry (\ref{extrasymm}), one obtains that for $D_{3}$ symmetric curve $\gamma=0$, hence:
\begin{equation}\label{d3curve}
\eta^{3}+\alpha\eta\zeta^{2}+\beta(\zeta^{6}-1)=0.
\end{equation}
%
\end{example}\vspace{2mm}
%
%
%
\begin{example}[\enf{Platonic monopoles}]
%
An interesting class is given by those monopoles which are invariant under the \enf{Platonic groups}; in these cases, Klein's theory of invariant polynomials proves very useful in implementing the symmetry requirements on the spectral curve. For instance, by symmetry considerations alone one can conclude that no \enf{octahedrically} symmetric monopole exists for $k=2$ and $k=3$; for $k=4$, it would have the following form:
\begin{equation}\label{oct}
\eta^{4}+a(\zeta^{8}+14\zeta^{4}+1)=0.
\end{equation}
Analogously, the simplest monopole curve with \enf{tetrahedral} symmetry is of the form (for $k=3$)
\begin{equation}\label{thetr}
\eta^{3}+ia\zeta(\zeta^{4}-1)=0.
\end{equation}
Notice that after a rotation, this curve becomes
\begin{equation}\label{thetr1}
\eta^{3}+a(\zeta^{6}+5\sqrt{2}\zeta^{3}-1)=0,
\end{equation}
thus exhibiting the $C_{3}$ symmetry around the $x_{3}$ axis (cf. eq. (\ref{c3curve}) ). The simplest curve with \enf{icosahedral} symmetry is (for $k=6$)
\begin{equation}\label{ico}
\eta^{6}+a\zeta(\zeta^{10}+11\zeta^{5}-1)=0.
\end{equation}
We remark that the curves (\ref{thetr}), (\ref{oct}), (\ref{ico}) only satisfy the reality conditions \huno: for them to describe monopoles, they also have to satisfy conditions \hdue\, and \htre. One can prove (see \cite{symmmon}), that the curves (\ref{thetr}), (\ref{oct}), are indeed spectral curves for monopoles of charge 3 and 4, for suitable values of $a$; on the other hand, there is no charge $6$ monopole with icosahedral symmetry.\\
Note that the quotients of the curves (\ref{thetr}), (\ref{oct}), (\ref{ico}) by the respective symmetry groups are \enf{elliptic curves}: this proved a great advantage in obtaining the above results. Indeed, the explicit solutions for the tetrahedral and icosahedral monopoles are expressed in terms of elliptic functions, and the constant $a$ in terms of elliptic periods.
\end{example}

These last examples are in fact paradigmatic of the general situation for symmetric monopoles: the symmetry, and reality conditions impose (sometimes stringent) constraints on the spectral curve, but this is not enough to conclude that the constrained curve does indeed correspond to a monopole. For this to be the case, conditions \hdue\,and \htre\,(or \ndue\, and \ntre\, in Nahm's formulation) need to be satisfied as well: this proves to be a very difficult step in general, as it involves relations between integrals on the spectral curve, which become harder to find explicitly the higher the genus of the curve. In the above cases, the spectral curve admits an elliptic quotient, so the integral reduce to hyperelliptic ones, which are manageable; we shall see that the same happens for a certain symmetric 3-monopole (cf. \cite{BE06} and section \ref{sec:be}). In the case of the cyclic 3-monopole, which is the object of the present work, the general quotient is hyperelliptic (cf. section \ref{sec:quotient}), which is a slightly more involved case.

%
%
%
%
%
%
%
%
%
